HVACMeter: Apportionment of HVAC Power to Thermal Zones and Air Handler Units

Heating, Ventilation and Air Conditioning (HVAC) systems consume almost half of the total energy use of commercial buildings. To optimize HVAC energy usage, it is important to understand the energy consumption of individual HVAC components at fine granularities. However, buildings typically only have aggregate building level power and thermal meters. We present HVACMeter, a system which leverages existing sensors in commercial HVAC systems to estimate the energy consumed by individual components of the HVAC system, as well by each thermal zone in buildings. HVACMeter can be generalized to any HVAC system as it uses the basic understanding of HVAC operation, heat transfer equations, and historical sensor data to estimate energy. We deploy HVACMeter to three buildings on our campus, to identify the set of sensors that are important for accurately disaggregating energy use at the level of each Air Handler Unit and each thermal zone within these buildings. HVACMeter power estimations have on an average 44.5 % less RMSE than that of mean power estimates. Furthermore, we highlight the usefulness of HVACMeter energy estimation model for a building fault detection application by quantifying the amount of energy that can be saved by fixing particular faults.

==> background.tex <==
\section{Background}
\label{sec:background}


==> conclusion.tex <==
\section{Conclusion}
Heterogeneity present in sensor names and metadata are an impediment
to development of reusable applications in large scale sensor
deployments. We present the scale and the describe the challenges in mapping sensors in
HVAC systems in our university buildings to a standardized naming
schema. Regular expression based methods can map sensors to their respective types but tend to be brittle
to minor variations in the sensor metadata and require substantial domain expertise. Our proposed framework,
Zodiac, uses hierarchical clustering for grouping the sensors based
on the inherent patterns in the sensor metadata. We applied hierarchical
clustering on four buildings in our campus, and the clusters
were grouped together based on sensor type with an average accuracy
of 98.5\%. Zodiac uses the clusters to train a random forest classifier
using active learning techniques. Our active learning algorithm labeled
sensors across three buildings to their respective types with
an average accuracy of 98\% requiring 27\% fewer ground truth labels
than regular expression based methods. Using uniform sensor
labels, we develop a simplified gray box energy model for Variable
Air Volume (VAV) boxes and Air Handler Units (AHUs) in
the HVAC system. Using pre-specified fault detection rules, we
detected 135 faults across five buildings with an estimated energy
impact of 127.2 MMBTU/year.




%\vspace{2mm}


==> faults_backup.tex <==
\section{Fault Analysis}

\begin{table*}[t!]\normalsize
\vspace{-0.2cm}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{1cm}p{8cm}p{4.5cm}p{2cm}p{2cm}}
%\multicolumn{1}{c}{\textbf{Index}} & \multicolumn{1}{c}{\textbf{Rules}} & \multicolumn{1}{c}{\textbf{Possible Fault}} & \multicolumn{1}{c}{\textbf{Detected Faults}} & \multicolumn{1}{c}{\textbf{Energy Loss}}\\%[0.1cm]
 \centering {\multirow{2}{*}{\textbf{Index}}} & \centering{ \multirow{2}{*}{ \textbf{Rules}}} &  \centering {\multirow{2}{*}{ \textbf{Possible Faults}}} & \multicolumn{1}{c}{\textbf{Detected Faults}} & \multicolumn{1}{c}{\textbf{Energy Loss}}\\%[0.1cm]
\multicolumn{1}{c}{}& \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(Number)} & \multicolumn{1}{c}{(MMBTU/Year)}\\[0.1cm]\hline\\[-0.1cm]

\parbox{1cm}{\centering 1}    & \parbox{8cm}{$Correlation(T_{MA, measured}, T_{MA, estimated}) < C_{th,1}$} & \parbox{4.5cm}{Economizer damper broken} & \parbox{2cm}{\centering 3} & \parbox{2cm}{\centering 59.45}\\[0.3cm]                   

\parbox{1cm}{\centering 2}     & \parbox{8cm}{When $C_{valve}=0$, $MPE(T_{SA, AHU}, T_{MA})< C_{th,2}$} & \parbox{4.5cm}{AHU cooling valve leaking} & \parbox{2cm}{\centering 1} & \parbox{2cm}{\centering 1.446}\\[0.3cm]                   

%\parbox{1cm}{\centering 3}     & \parbox{8cm}{When $C_{valve}=100$, $T_{AH}>0.9\cdot T_{MA}$ } & \parbox{4.5cm}{AHU cooling valve stuck} & \parbox{2cm}{\centering 4} & \parbox{2cm}{\centering N/A}\\[0.3cm]                   

\parbox{1cm}{\centering 4}     & \parbox{8cm}{When $H_{valve,AHU}=0$, $MPE(T_{SA, AHU}, T_{MA})>C_{th,3}$} & \parbox{4.5cm}{AHU heating valve leaking} & \parbox{2cm}{\centering 1} & \parbox{2cm}{\centering 0.1111}\\[0.3cm]                   

%\parbox{1cm}{\centering 5}     & \parbox{8cm}{When $H_{valve,AHU}=100$, $T_{SA, AHU}<1.1\cdot T_{MA}$} & \parbox{4.5cm}{AHU heating valve stuck} & \parbox{2cm}{\centering 2} & \parbox{2cm}{\centering N/A}\\[0.3cm]                   

%\parbox{1cm}{\centering 6}     & \parbox{8cm}{$ (C_{valve}>0)$  $\&$  $(H_{valve, AHU}>0)$} & \parbox{4.5cm}{Simultaneous heating and cooling} & \parbox{2cm}{\centering 1} & \parbox{2cm}{\centering N/A}\\[0.3cm]                   
                                                                                                          
%\parbox{1cm}{\centering 7}     & \parbox{8cm}{$RMSPE(T_{supply, AHU}, TS_{supply, AHU}) >C_{th,4}$ } & \parbox{4.5cm}{Heating or cooling valve stuck} & \parbox{2cm}{\centering 13} & \parbox{2cm}{\centering N/A}\\[0.3cm]       

%\parbox{1cm}{\centering 8}     & \parbox{8cm}{When $H_{valve, VAV}<0$, $MPE(T_{SA, VAV}, T_{AH})>C_{th,5}$} & \parbox{4.5cm}{VAV heating valve leaking} & \parbox{2cm}{\centering 6} & \parbox{2cm}{\centering N/A}\\[0.3cm]                   

\parbox{1cm}{\centering 9}     & \parbox{8cm}{If $unoccupied$ $\&$ $(T_{zone}<T_{upper limit})$, $q_{vav}> 1.1\cdot q_{min}$} & \parbox{4.5cm}{Configuration error} & \parbox{2cm}{\centering 5} & \parbox{2cm}{\centering 4.579}\\[0.3cm]       

\parbox{1cm}{\centering 10}   & \parbox{8cm}{$RMSPE(q_{vav}, qs_{vav}) >C_{th,6}$ } & \parbox{4.5cm}{VAV damper leaking or stuck} & \parbox{2cm}{\centering 99} & \parbox{2cm}{\centering 61.66}\\[0.3cm]   \hline\\[-0.1cm]

\multicolumn{5}{l}{\parbox{15cm}{
\begin{tabular}{l l l l }
T=Temperature, & TS=Temperature Setpoint, & SA=Supply Air, & MA = Mixed Air, \\
$C_{valve}$=Cooling Valve Command, & $H_{valve}$=Heating Valve Command, & $C_{th}$=Threshold &  OC=Occupied Command, \\
AHU=Air Handler Unit, & VAV=Variable Air Volume, & RMSPE=Root Mean Square Percentage Error, & MPE = Mean Percentage Error, \\
corr=Correlation, & q=Supply Flow, & qs = Supply Flow Setpoint \\
\end{tabular}
}
}\\
\end{tabular}
}
    \caption{Fault Detection Rules and Result} 
    \vspace{-0.1Cm}
    \label{tab:faultrules}
\end{table*}



\begin{figure}[Ht]
\includegraphics[width=3in]{figs/SAFNotMatch_EBU1VAV7305-1.pdf}
\vspace{-3mm}
\caption{Supply air flow does not match its setpoint}
\label{fig:flow_fault}
\vspace{-3mm}
\end{figure}

\begin{figure}[Ht]
\includegraphics[width=3in]{figs/EconomizerDamper_EBU1AH22.pdf}
\vspace{-3mm}
\caption{Economizer damper does not work properly}
\label{fig:econ_fault}
\vspace{-3mm}
\end{figure}

HVAC systems are designed with care to meet usage requirements and be energy efficient. However, faults develop over time, and facilities managers struggle to maintain the HVAC systems~\cite{mills2010building}. For example, across the 55 buildings managed by a single BMS on our campus, it is common to have over 100,000 outstanding faults, and more than 10,000 fault alarms are generated \emph{per day}. Lack of standard point naming convention is one of the stumbling blocks for adoption of advanced detection and prioritization algorithms~\cite{schumann2011adaptable}, and we present fault detection as an example application to show the benefits of standardized point naming.

We detect specific types of faults in AHUs and VAVs that are known to be common by facilities managers, and are not detected by fault detection techniques used by BMS. We use rule based detection methods, as they are supported by many fault detection frameworks~\cite{skyspark}, and can be designed to accurately detect any type of fault. Table \ref{tab:faultrules} lists the type of faults we detect and a summary of the rule used for detection.

%With time, faults develop across the system, and facilities managers rely on sensor data and the analysis provided by Building Management System (BMS) to detect these faults and fix them. 
%Focus on specific type of faults which are common in our campus. Use the point type and equipment type mapping learnt from previous part.

The generic methodology we use is to estimate the ideal values for a parameter, and compare it with measured values for that parameter. For some faults, the estimation is easy, as there points that indicate the setpoint for a particular sensor. For example, measured supply air flow should be close to its setpoint. For other faults, we use data from sensors and knowledge about HVAC working for detection. For example, we can check if the economizer damper is working correctly if the mixed air temperature changes with changes in damper position. We estimate the mixed air temperature by using measured return air temperature, outside air temperature, and economizer damper position, which determines the proportion of outside air and return air in the mixer. We can compare this estimated value to the measured mixed air temperature for detecting faults. However, it is common for temperature sensors to develop minor drifts over time, so to detect damper faults more accurately we check the correlation between the measured and estimated mixed air temperature. When they are not correlated, either one of the sensors is incorrect, or the outside air damper is damaged. Figure \ref{fig:econ_fault} shows an example of a fault detected using this metric, and we can see that the observed mixed air temperature does not change as expected with changes in economizer damper position.

To reduce false positives, and to ensure we detect faults which cause significant wastage or discomfort, we use conservative thresholds in our rules and only identify faults that persist for extended periods of time. We ignore transient and minor faults as facilities management does not have enough manual labor to fix minor faults that occur across 55 buildings. Figure \ref{fig:flow_fault} shows an example of supply air flow fault detected using our rules, and we can observe that the air flow is almost zero even when the setpoint is set to 300 cfm. We detected total of 135 faults \BB{change}, and we manually verified all of these faults and 83.7\% \BB{change} of these were correctly identified. The errors in detection occurred when the thresholds were not conservative enough for certain conditions, which perhaps points towards using data driven fault detection methods.

In addition, to help prioritize the faults that cause egregious wastage, we estimate the energy impact of faults using the simplified energy model we presented in Sections \ref{sec:cooling} and \ref{sec:heating}. We estimate energy for those faults whose ideal values can be estimated to compare the energy consumption between the faulty and operating conditions. We calculate savings based on at least one week of data and extrapolate the savings for a year based on correlation with outdoor weather conditions. Table \ref{tab:faultrules} summarizes the faults detected and their energy wastage. 

